Attentive Walk-Aggregating Graph Neural Networks

Graph neural networks (GNNs) have been shown to possess strong representation power, which can be exploited for downstream prediction tasks on graph-structured data, such as molecules and social networks. They typically learn representations by aggregating information from the $K$-hop neighborhood of individual vertices or from the enumerated walks in the graph. Prior studies have demonstrated the effectiveness of incorporating weighting schemes into GNNs; however, this has been primarily limited to $K$-hop neighborhood GNNs so far. In this paper, we aim to design an algorithm incorporating weighting schemes into walk-aggregating GNNs and analyze their effect. We propose a novel GNN model, called AWARE, that aggregates information about the walks in the graph using attention schemes. This leads to an end-to-end supervised learning method for graph-level prediction tasks in the standard setting where the input is the adjacency and vertex information of a graph, and the output is a predicted label for the graph. We then perform theoretical, empirical, and interpretability analyses of AWARE. Our theoretical analysis in a simplified setting identifies successful conditions for provable guarantees, demonstrating how the graph information is encoded in the representation, and how the weighting schemes in AWARE affect the representation and learning performance. Our experiments demonstrate the strong performance of AWARE in graph-level prediction tasks in the standard setting in the domains of molecular property prediction and social networks. Lastly, our interpretation study illustrates that AWARE can successfully capture the important substructures of the input graph. The code is available on $\href{https://github.com/mehmetfdemirel/aware}{GitHub}$.

==> main_theory.tex <==
%\vspace{-0.5em}
\section{Theoretical Analysis}
%\vspace{-0.5em}
\label{sec:analysis}
\YL{remove the space-saving commands like  vspace since we don't have space  limitation}

\YL{Need to move the Appendix A.1-A.3 to the main body in the journal version; only keep in the appendix A.4-A.5 which are just tools from existing work. Similarly, move needed details in other sections to the main body; only keep minor details in the appendix.}



For the design of our walk-aggregation GNN with weighting schemes, we are interested in the following two fundamental questions: \emph{What representation can it obtain? Under what conditions can the weighting scheme improve the prediction performance?}
This section analyzes the weighting $\mathbf{S}_{ij} = S(f_i, f_j)$ for these two questions.%
\footnote{For the other weighting schemes $\Wv$ and $\Wg$, we know $\Wv$ weights the vertex embeddings $f_i$, and $\Wg$ weights the final embeddings $F_{(n)}$, emphasizing important directions in the corresponding space. If $\Wv$ has singular vector decomposition $\Wv = U\Sigma V^\top$, then it will relatively emphasize the singular vector directions with large singular values. Similar for $\Wg$. See~\Cref{sec:interpretation} for some visualization.} 
We assume: 
\begin{itemize}[topsep=0pt,itemsep=0pt,partopsep=0pt,parsep=0pt]
    \item  $\Wv = \Wg = I$, the number of attributes is $C=1$, and the activation is linear $\sigma(z) = z$.   
\end{itemize} 
Here, the assumptions simplify the notations, and allow focusing on the effect of $\mathbf{S}_{ij}$. \Cref{app:general_analysis} presents an analysis for more general $\Wv, \Wg$ and $C>1$.

%We will show that our algorithm incorporates the weighting scheme in a principled way, and thus can potentially highlight important information and reduce irrelevant information for the prediction, which can improve learning. 
%To this end, we will first show that the graph embedding $f_{(n)}$ is a linear mapping of a high dimension vector $\Lambda_{(n)} c_{(n)}$ into the low dimension embedding space, where the vector $c_{(n)}$ records the statistics about the walks in the graph and $\Lambda_{(n)}$ is a diagonal weighting matrix depending on $\mathbf{S}$. 
We will show that the weighting scheme can highlight important information, and reduce irrelevant information for the prediction, and thus improve learning. 
To this end, we first analyze what information can be encoded in our graph representation, and how they are weighted (Theorem~\ref{thm:rep}). We then examine why the weighting can help learning a predictor with better performance (Theorem~\ref{thm:learn}). 
We focus on the intuition and implications here, and present proofs and more discussion in \Cref{app:analysis}.
 
\mypara{Weighted representation in {\AWARE}.} 
%The unweighted version of our model has been analyzed in~\citep{liu2019n}, which shows that the representation is a linear mapping of the so-called count statistics of the input graph. However, with the weighting scheme, their analysis does not hold. Fortunately, we are able to introduce a variant of the count statistics and show a similar result. 
We first formally define the walk information in the graph, and a notion of walk weights (which will be shown to be exactly the weights induced by our method). Recall that we assume the number of attributes is $C=1$. $K$ is the number of possible attribute values, and the columns of $W \in \mathbb{R}^{r\times K}$ are embeddings for different attribute values $u$. Let $W(u)$ denote the column for value $u$, i.e., $W(u) = W h(u)$ where $h(u)$ is the one-hot vector of $u$.  

\begin{definition}[Walk Statistics] \label{def:walkstat}
A \emph{walk type} of length $n$ is a sequence of $n$ attribute values $v = (v_1, v_2, \cdots, v_n)$.
The \emph{walk statistics} vector $c_{(n)}(G) \in \mathbb{R}^{K^n}$ is the histogram of all walk types of length $n$ in the graph $G$, i.e., each entry is indexed by a walk type $v$ and the entry value is the number of walks with the attribute values $v$ in the graph. 
Furthermore, let $c_{[T]}(G)$ be the concatenation of $c_{(1)}(G), \dots, c_{(T)}(G)$. When $G$ is clear from the context, we write $c_{(n)}$ and $c_{[T]}$ for short. 
\end{definition} 

% We also introduce the following notions for describing the linear mapping projecting $c_{(n)}$ to the representation $f_{(n)}$. 

% \begin{definition}[$\ell$-way Column Product]  
% $W^{[n]}$ is an $r$ by $K^n$ matrix, whose columns are indexed by walk types $v = (v_1, v_2, \cdots, v_n)$ and equal  $W(v_1) \odot W(v_2) \odot \cdots \odot W(v_{n})$.
% \end{definition}

% \YL{may use $\lambda(v)$ to denote the weight, to be consistent with $\Lambda$, and distinguish from $W$}
\begin{definition}[Walk Weights] \label{def:weight}
The weight of a walk type $v = (v_1,\ldots, v_{n})$ is 
$ %\begin{align*}
    \lambda(v) := \prod_{i=1}^{n-1} S(W(v_i), W(v_{i+1})) 
$ %\end{align*}
where $S(\cdot, \cdot)$ is the weight function in Eq~\eqref{eq:score}.
\end{definition}


We have the following theorem which shows that our representation is a linear mapping of the weighted walk statistics.

\begin{theorem} \label{thm:rep}
The embedding $f_{(n)}$ is a linear mapping of the walk statistics $c_{(n)}$: 
\begin{align*}
    f_{(n)} = \mathcal{M}_{(n)} \Lambda_{(n)} c_{(n)}
\end{align*}
where $\mathcal{M}_{(n)}$ is a matrix depending only on $W$, and $\Lambda_{(n)}$ is a $K^n$-dimensional diagonal matrix whose columns are indexed by walk types $v$, and have diagonal entries $\lambda(v)$.
Therefore, $ f_{[T]} := \mathcal{M}\Lambda c_{[T]} $
where $\mathcal{M}$ is a block-diagonal matrix with diagonal blocks $\mathcal{M}_{(1)}, \mathcal{M}_{(2)}, \ldots, \mathcal{M}_{(T)}$, and $\Lambda$ is block-diagonal with blocks $\Lambda_{(1)}, \Lambda_{(2)}, \ldots, \Lambda_{(T)}$.
\end{theorem}

In words, $c_{(n)}$ is first weighted by our weighting scheme where the count of each walk type $v$ is weighted by the corresponding walk weight $\lambda(v)$, and then compressed from the high dimension $\mathbb{R}^{K^n}$ to the low dimension $\mathbb{R}^{r}$. Ideally, we would like to have relatively larger weights on walk types important for the prediction task and smaller for those not important. This provides the basis for the focus of our analysis: the effect of weighting for the learning performance. 
%The weighted walk statistics is then compressed from a high dimension to a low dimension by multiplying with $W^{[n]}$. It is well known in the compressive sensing literature that when $W^{[n]}$ satisfies the Restricted Isometry Property (RIP) on the sparse vectors $\Lambda_{(n)} c_{(n)}$, then $\Lambda_{(n)} c_{(n)}$ can be recovered from $f_{(n)}$, i.e., $f_{(n)}$ preserve the information of $\Lambda_{(n)} c_{(n)}$. The appendix provides a formal proof (Theorem~\ref{thm:compressive}) that for a wide family of $W$, $W^{[n]}$ satisfies RIP on $\Lambda_{(n)} c_{(n)}$, and thus $\mathcal{M}$ satisfies RIP on $\Lambda c_{[T]}$.
 

%To focus on the effect of the weighting, we will make the following simplifying assumption that $\mathcal{M}$ satisfies the requirement of compressive sensing: $\mathcal{M}$ satisfies the $(2s,\epsilon)$-RIP, and $c_{[T]}$ is $s$-sparse.

% Once we have shown $f_{[T]} := \mathcal{M}\Lambda c_{[T]}$ and $\mathcal{M}$ can satisfy RIP, we are now ready to analyze if the weighting  $\Lambda$ can potentially improve the learning of a predictor on $f_{[T]}$.

% The intuition for the benefit of appropriate weighting is simple. Suppose that the label is given by a linear function on $c_{[T]}$ with parameter $\theta^*$, i.e., $y = \langle \theta^*, c_{[T]}\rangle$. When we learn over the weighted features $\Lambda c_{[T]}$, if the support of the diagonal entries $\textrm{diag}(\Lambda)$ contains the support of $\theta^*$ (i.e., if $\theta^*_i \neq 0$ then $\Lambda_{ii} \neq 0$), the parameter $\Lambda^\dagger\theta^*$ on $\Lambda c_{[T]}$ has the same predictions and loss as $\theta^*$ on $c_{[T]}$. So we only need to learn $\Lambda^\dagger\theta^*$ on $\Lambda c_{[T]}$, which can require fewer data samples for learning (equivalently, smaller loss for a fixed amount of samples).
% Learning over $f_{[T]}$ is learning over a compressed version of $\Lambda c_{[T]}$, which shares the same intuition. 

% To formalize the intuition, we consider the binary classification task with the logistic loss function $\ell(g, y) = \log(1+\exp(-gy))$ where $g$ is the prediction and $y$ is the true label. Let $\ell_\mathcal{D}(\theta) = \mathbb{E}_{\mathcal{D}} [ \ell(g_\theta, y)]$ 
% denote the risk of a linear classifier $g_\theta$ with a parameter vector $\theta$ over the data distribution $\mathcal{D}$. Let $\theta^*$ denote the parameter of the classifier over $c_{[T]}$ minimizing $\ell_\mathcal{D}$.
% Suppose we have a dataset $\{(G_i, y_i)\}_{i=1}^M$ i.i.d.\ sampled from $\mathcal{D}$, and $\hat{\theta}$ is the parameter over $ f_{[T]}(G)$ which is learned via $\ell_2$-regularization with regularization coefficient $\lambda$:
% \begin{align}
% \hat{\theta} = \arg\min_{\theta}  \frac{1}{M} \sum_{i=1}^M \ell\Big(\langle \theta,  f_{[T]}(G_i) \rangle, y_i\Big)  + \lambda \| \theta \|_2.
% \end{align}

% \YL{update the theorem by taking into account the weight learning process. Use a net argument for the weight of the representation model, and then apply this to each of the model in the net and get the guarantee on the net; then use Lipschitz argument. Can assume that the representation is normalized before feeding into classifiers.}
% \begin{theorem}  \label{thm:weighted_linear}
% Assume that $\mathcal{M}$ satisfies the $(2s,\epsilon)$-RIP, and $c_{[T]}$ is $s$-sparse. Also assume that the support of $\textrm{diag}(\Lambda)$ contains the support of $\theta^*$. For any $\delta \in (0,1)$, the $\hat{\theta}$ minimizing the $\ell_2$-regularized logistic loss over the embeddings $f_{[T]}(G_i)$'s satisfies with probability at least $1-\delta$:
% \begin{align}
% \ell_{\mathcal{D}}(\hat{\theta}) \le \ell_{\mathcal{D}}(\theta^*) + O\left( B_\Lambda \sqrt{\epsilon + \frac{1}{M}\log\frac{1}{\delta} } \right)
% \end{align} 
% for an appropriate choice of regularization coefficient $\lambda$.
% Here the term $B_\Lambda$ is defined as
% \begin{align}
%     B_\Lambda := \|\Lambda^{\dagger}\theta^*\|_2 \max_{G \sim \mathcal{D}} \|\Lambda c_{[T]}(G)\|_2
% \end{align}
% and $\Lambda^{\dagger}$ is the pseudo-inverse of $\Lambda$.
% \end{theorem}

%Once we have shown that the embedding $f_{(n)}$ can be viewed as a linear mapping of the weighted walk statistics to low dimensional representations, we are now ready to analyze if the weighting can potentially improve the learning.


%To focus on the effect of the weighting, we will make the following simplifying assumption that $\mathcal{M}$ satisfies the requirement of compressive sensing: $\mathcal{M}$ satisfies the $(2s,\epsilon)$-RIP, and $c_{[T]}$ is $s$-sparse. Note that the RIP can also be satisfied easily (e.g., setting $W$ to have independent Rademacher entries and have large enough dimensions, and $\Ww$ can be arbitrary). In practice, our method is more general and the parameters are learned over the data. Still, the analysis in the special case under the assumptions can provide useful insights for understanding our method, in particular, how the weighting can affect the learning of a predictor over the embeddings. 


%\mypara{The Effect of Weighting on Learning.}
\mypara{Learning guarantees of {\AWARE}.}
%The intuition for the benefit of appropriate weighting is simple. 
To illustrate the effect of weighting, suppose the label is given by a linear function on $c_{[T]}$ with parameter $\beta^*$, i.e., $y = \langle \beta^*, c_{[T]}\rangle$. First, consider learning a linear function over the weighted features $\Lambda c_{[T]}$.  If $\Lambda$ is invertible, the parameter $\Lambda^{-1}\beta^*$ on $\Lambda c_{[T]}$ has the same output  as $\beta^*$ on $c_{[T]}$, and thus has the same loss. So, we only need to learn $\Lambda^{-1}\beta^*$. The sample size needed will depend on the factor $\|\Lambda^{-1}\beta^*\|_2 \|\Lambda c_{[T]}\|_2$, which is potentially smaller than $\|\beta^*\|_2 \| c_{[T]}\|_2$ for the unweighted case. This means fewer data samples are needed (equivalently, smaller loss for a fixed amount of samples).

Now, consider the case of learning over $f_{[T]}(G) = \mathcal{M}\Lambda c_{[T]}$ that has an extra $\mathcal{M}$ (defined in Theorem~\ref{thm:rep}). We note that $c_{[T]}$ can be sparse compared to its high dimension (since only a very small fraction of all possible walk types will likely appear in a graph). Well-established results from compressive sensing show that when $\mathcal{M}$ has the Restricted Isometry Property (RIP), learning over $\mathcal{M}\Lambda c_{[T]}$ is comparable to learning over $\Lambda c_{[T]}$. Indeed, Theorem~\ref{thm:compressive} in Appendix~\ref{app:analysis} shows when $W$ is random and the embedding dimension $r$ is large enough, there are families of distributions of $W$ such that $\mathcal{M}$ has RIP for $\Lambda c_{[T]}$. Thus, we assume $\mathcal{M}$ has RIP, and focus on the analysis of how $\Ww$ affects the weighting and the learning.  

However, the above intuition is only for learning over a \emph{fixed} weighting $\Lambda$ induced by a \emph{fixed} $\Ww$, while in fact $\Ww$ needs to be \emph{learned}. Our key challenge is to incorporate the learning of $\Ww$ in the analysis.  
Formally, we consider learning $\Ww$ from a hypothesis class $\Wfamily$, and let $\Lambda(\Ww)$ and $f_{[T]}(G; \Ww)$ denote the weights and representation given by $\Ww$. 
For prediction, we consider binary classification with the logistic loss $\ell(g, y) = \log(1+\exp(-gy))$ where $g$ is the prediction and $y$ is the true label. 
Let $\ell_\mathcal{D}(\theta, \Ww)$ be the risk of a linear classifier with a parameter $\theta$ on $f_{[T]}(G; \Ww)$ over the data distribution $\mathcal{D}$.
Given $M$ i.i.d.\ samples $\{(G_i, y_i)\}_{i=1}^M$ from $\mathcal{D}$, consider learning over ${\Ww \in \Wfamily, \|\theta\|_2\le B_\theta}$ for a regularization coefficient $B_\theta$: 
\begin{align*}
\hat{\theta}, \widehat{\Ww} = \arg\min  \frac{1}{M} \sum_{i=1}^M \ell\Big(\langle \theta,  f_{[T]}(G_i; {\Ww}) \rangle, y_i\Big).
\end{align*}

To derive error bounds, suppose $\Wfamily$ is equipped with a norm $\|\cdot\|$ and let $\mathcal{N}(\Wfamily, \epsilon)$ be the $\epsilon$-covering number of $\Wfamily$ w.r.t.\ the norm $\| \cdot\|$ (other complexity measures on $\Wfamily$, such as VC-dimension, can also be used). 
Furthermore, let $\beta^*$ denote the best linear classifier on $ c_{[T]}$, and let $\ell^*_{\mathcal{D}}$ denote its risk.

% \begin{theorem}~\label{thm:learn}
% Assume that $\mathcal{M}$ satisfies the $(2s,\epsilon)$-RIP, and $c_{[T]}$ is $s$-sparse. Assume that $\Lambda$ is invertible and $f_{[T]}(G; \Ww)$ is $L_f$-Lipschitz. For any $\delta \in (0,1)$ and $\epsilon \in (0,1)$, there exists an appropriate choice of regularization coefficient $B_\theta$, such that if the sample size
% \begin{align*}
%     M \ge O\left(  \frac{1}{\epsilon^2}\left(rT +  \log\frac{1}{\delta}  +  \log \mathcal{N}\left(\Wfamily, \frac{\epsilon }{32 B_\theta L_f} \right) \right)   \right),
% \end{align*}
% then with probability at least $1-\delta$,
% \begin{align*}
% & \quad \ell_{\mathcal{D}}(\hat{\theta}, \widehat{\Ww})  \le \ell^*_{\mathcal{D}} + \epsilon + \min_{\Ww \in \Wfamily} B(\Ww) \times  O\left( \sqrt{ \epsilon_0 + \epsilon^2} \right)
% \end{align*}  
% where the term $B(\Ww)$ is defined as
% \begin{align*}
%     B(\Ww) := \|\Lambda(\Ww)^{-1}\beta^*\|_2 \times \max_{G \sim \mathcal{D}} \|\Lambda(\Ww) c_{[T]}(G)\|_2.
% \end{align*} 
% \end{theorem} 
\begin{theorem}~\label{thm:learn}
Assume $c_{[T]}$ is $s$-sparse, $\mathcal{M}$ satisfies $(2s,\epsilon_0)$-RIP, $\Lambda(\Ww)$ is invertible and $f_{[T]}(G; \Ww)$ is $L_f$-Lipschitz over $\Wfamily$. For any $\delta, \epsilon \in (0,1)$, there are regularization coefficient values $B_\theta$ such that with probability $\ge 1-\delta$:
\begin{align*}
&  \ell_{\mathcal{D}}(\hat{\theta}, \widehat{\Ww})  \le \ell^*_{\mathcal{D}} + 2 \epsilon  +  O\left( \sqrt{\frac{r T + \mathcal{C}_\epsilon(\mathcal{W})   }{M} } \right)  + \min_{\Ww \in \Wfamily} B(\Ww) \times O\left(  \sqrt{\epsilon_0 + \frac{  \mathcal{C}_\epsilon(\mathcal{W})}{M}  }  \right)  
\end{align*}  
where $\mathcal{C}_\epsilon(\mathcal{W}) := \log \mathcal{N}\left(\Wfamily, \frac{\epsilon }{8 B_\theta L_f} \right) + \log\frac{1}{\delta}$, and
\begin{align*}
    B(\Ww) :=  \max_{G \sim \mathcal{D}} \|\Lambda(\Ww) c_{[T]}(G)\|_2 \|\Lambda(\Ww)^{-1}\beta^*\|_2.
\end{align*} 
\end{theorem}

\textit{Remark.} \Cref{thm:learn} shows that the learned model has risk comparable to that of the best linear classifier on the walk statistics, given sufficient data. Let's now compare to the unweighted case (i.e., $\Lambda$ is the identity matrix), where $\log \mathcal{N}\left(\Wfamily, \frac{\epsilon }{8 B_\theta L_f} \right)$ reduces to 0, and $B(\Ww)$ reduces to  
$ %\begin{align}
    B_0 :=   \max_{G \sim \mathcal{D}} \|c_{[T]}(G)\|_2 \|\beta^*\|_2.
$ %\end{align} 
So, our method needs extra samples to learn $\Ww$, leading to the extra error terms related to $ \log \mathcal{N}\left(\Wfamily, \frac{\epsilon }{8 B_\theta L_f} \right)$. 
On the other hand, the benefit of weighting is replacing the factor $B_0$ with $\min_{\Ww} B(\Ww)$. If there is $\Ww^*$ with $B(\Ww^*) \ll B_0$, the error is significantly reduced. Therefore, there is a trade-off between the reduction of error for learning classifiers on an appropriate weighted representation and the additional samples needed for learning an appropriate weighting. When the labels indeed depend on some important walks rather than on all walks, the weighting can alleviate the problem of over-squashing shown in~\citet{alon2020bottleneck}.

Our analysis also reveals that weighting is not panacea: its ability to improve learning depends on (1) whether it can assign the large weights to important features, and (2) \emph{whether the benefit of weighting important features exceeds the overhead of learning a proper weighting scheme}. (1) is generally accepted while (2) is largely overlooked (at least not explicitly discussed) in existing studies.


\textit{An illustrative example.} The benefit of weighting can be significant in practice. $\min_{\Ww} B(\Ww)$ can be much smaller than $B_0$, especially when some features (i.e., walk types) in $c_{[T]}$ are important while others are not, which is true for many real-world applications.
Suppose $c_{[T]}(G)$ is $s$-sparse with each non-zero entry being some constant $c$. Suppose only a few of the features are useful for the prediction, i.e., $\beta^*$ is $\rho$-sparse with each non-zero entry being some constant $b$, and $\rho \ll s$. Suppose there is a weighting $\Ww^*$ that leads to weight $\Upsilon$ on the entries corresponding to the $\rho$ important features (i.e., the non-zero entries in $\beta^*$), and weight $\upsilon$ for the other features where $|\upsilon| \ll |\Upsilon|$.
Then it can be shown that
$ %\begin{align*}
    \frac{\underset{\Ww}{\min} B(\Ww)}{B_0} \le   \sqrt{\frac{\rho}{s} + \left(1 -\frac{\rho}{s}\right) \left(\frac{\upsilon}{\Upsilon} \right)^2}.
$ %\end{align*}
Since $\rho \ll s$ and $|\upsilon| \ll |\Upsilon|$, $\underset{\Ww}{\min}\; B(\Ww)$ is much smaller than $B_0$, so the weighting can significantly reduce the error. 

This example demonstrates that with a proper weighting that highlights important features and depresses irrelevant ones for prediction, the error can be much smaller than the error without weighting. If this benefit exceeds the overhead in learning the proper weighting, the learning performance is improved. This trade-off is indeed visible on many datasets; see our experimental results in Section~\ref{sec:experiments}. 
The analysis also shows that a trained {\AWARE} model finds a weighting that automatically highlights important substructures like edges in the graph and provide useful interpretation; see the interpretation study in Section~\ref{sec:interpretation}.

==> tables/ablation1.tex <==
\newfloatcommand{capbtabbox}{table}[][0.58\textwidth]

\begin{figure}
\begin{floatrow}
\capbtabbox{%
\resizebox{\linewidth}{!}{
    \begin{tabular}{l c c c c}
        \toprule
        \textbf{Task} & \textbf{No} \bm{$\Wv$} & \textbf{No} \bm{$\Ww$} & \textbf{No} \bm{$\Wg$} & \textbf{No} \bm{$\Wv$}, \bm{$\Ww$} \textbf{or} \bm{$\Wg$} \\
        \toprule
        \textsc{IMDB-BINARY} & $-5.03\%$ & $+1.12\%$ & $-1.96\%$ & $-7.54\%$ \\
        \midrule
        \textsc{NR-AR} & $+1.32\%$ & $-0.76\%$ & $+0.67\%$ & $+0.37\%$ \\
        \textsc{CT\_TOX} & $-9.00\%$ & $-2.09\%$ & $+0.70\%$ & $-3.07\%$ \\
        \textsc{FDA\_APPROVED} & $-7.83\%$ & $-2.39\%$ & $+1.38\%$ & $-4.16\%$ \\
        \textsc{MUV-466} & $-20.08\%$ & $-16.70\%$ & $-7.44\%$ & $+1.80\%$ \\
        \midrule
        \textsc{Delaney} & $-28.45\%$ & $-0.18\%$ & $-4.69\%$ & $-57.80\%$  \\
        \textsc{Malaria} & $-0.83\%$ & $+2.10\%$ & $-1.15\%$ & $-2.32\%$ \\
        \textsc{QM7} & $-11.59\%$ & $+3.74\%$ & $-18.45\%$ & $-71.39\%$ \\
        % \textsc{QM8} & \textsc{E1-CC2} & MAE & $-48.73\%$ & $-4.94\%$ & $-8.62\%$ & $+11.16\%$ \\
        % \midrule
        \bottomrule
    \end{tabular}
   }
}{%
  \caption{Change in performance on removing weighting components of {\AWARE}. ``+"\ /\ ``-" indicate relative improvement/decrease in performance with respect to the full {\AWARE} model respectively.} \label{tab:ablation1_performance_parts_removed}
}
\centering
    \ffigbox[0.36\textwidth]
    {
    \includegraphics[width=0.95\linewidth]{figures/interpret/NR-AR.pdf}
    }
    {
  \caption{Interpretation of graph-level attention $W_g$ for the \textsc{NR-AR} classification task.}%
  \label{fig:interpret_Wg}
}
\end{floatrow}
\end{figure}



% \begin{table}[t!]
%     \centering
%     \vspace{-1em}
%     \caption{Change in performance on removing weighting components of {\AWARE}. ``+"\ /\ ``-" indicate relative improvement/decrease in performance with respect to the full {\AWARE} model respectively.
%     }
%     \resizebox{0.8\textwidth}{!}{
%     \begin{tabular}{l c c c c}
%         \toprule
%         \textbf{Task} & \textbf{No} \bm{$\Wv$} & \textbf{No} \bm{$\Ww$} & \textbf{No} \bm{$\Wg$} & \textbf{No} \bm{$\Wv$}, \bm{$\Ww$} \textbf{or} \bm{$\Wg$} \\
%         \toprule
%         \textsc{IMDB-BINARY} & $-5.03\%$ & $+1.12\%$ & $-1.96\%$ & $-7.54\%$ \\
%         \midrule
%         \textsc{NR-AR} & $+1.32\%$ & $-0.76\%$ & $+0.67\%$ & $+0.37\%$ \\
%         \textsc{CT\_TOX} & $-9.00\%$ & $-2.09\%$ & $+0.70\%$ & $-3.07\%$ \\
%         \textsc{FDA\_APPROVED} & $-7.83\%$ & $-2.39\%$ & $+1.38\%$ & $-4.16\%$ \\
%         \textsc{MUV-466} & $-20.08\%$ & $-16.70\%$ & $-7.44\%$ & $+1.80\%$ \\
%         \midrule
%         \textsc{Delaney} & $-28.45\%$ & $-0.18\%$ & $-4.69\%$ & $-57.80\%$  \\
%         \textsc{Malaria} & $-0.83\%$ & $+2.10\%$ & $-1.15\%$ & $-2.32\%$ \\
%         \textsc{QM7} & $-11.59\%$ & $+3.74\%$ & $-18.45\%$ & $-71.39\%$ \\
%         % \textsc{QM8} & \textsc{E1-CC2} & MAE & $-48.73\%$ & $-4.94\%$ & $-8.62\%$ & $+11.16\%$ \\
%         % \midrule
%         \bottomrule
%     \end{tabular}
%     }
%     \label{tab:ablation1_performance_parts_removed}
% \end{table}

% \begin{table}[t!]
%     \centering
%     \vspace{-1em}
%     \caption{Change in performance on removing weighting components of {\AWARE}. ``+"\ /\ ``-" indicate relative improvement/decrease in performance with respect to the full {\AWARE} model respectively.}
%     \resizebox{0.8\textwidth}{!}{
%     \begin{tabular}{c c c c c c c}
%         \hline
%         Dataset & Task & Metric & No $\Wv$ & No $\Ww$ & No $\Wg$ & No $\Wv$, $\Ww$ or $\Wg$ \\
%         \toprule
%         \textsc{Delaney} &\textsc{Delaney} & RMSE & $-16.74\%$ & $+1.32\%$ & $-1.31\%$ & $-51.29\%$  \\
%         \textsc{Malaria} & \textsc{Malaria} & RMSE & $-2.19\%$ & $+1.91\%$ & $-1.03\%$ & $-2.78\%$ \\
%         \textsc{QM7} & \textsc{QM7} & MAE & $-0.06\%$ & $+4.91\%$ & $-12.74\%$ & $-72.85\%$ \\
%         % \textsc{QM8} & \textsc{E1-CC2} & MAE & $-44.59\%$ & $-1.35\%$ & $-5.40\%$ & $+16.22\%$ \\
%         % \midrule
%         \textsc{ClinTox} & \textsc{CT\_TOX} & ROC & $-3.20\%$ & $-1.64\%$ & $+1.31\%$ & $-4.43\%$ \\
%         \textsc{ClinTox} & \textsc{FDA\_APPROVED} & ROC & $-3.00\%$ & $-3.11\%$ & $-0.46\%$ & $-1.72\%$ \\
%         \textsc{Tox21} & \textsc{NR-AR} & ROC & $+1.71\%$ & $-0.16\%$ & $-0.45\%$ & $+1.29\%$ \\
%         % \textsc{MUV} & \textsc{MUV-466} & ROC & $-14.32\%$ & $-9.77\%$ & $-1.96\%$ & $+10.05\%$ \\
%         \bottomrule
%     \end{tabular}
%     }
%     \label{tab:ablation1_performance_parts_removed}
% \end{table}


% supervised N-gram values
% delaney 0.9256
% malaria 1.0931
% qm7 71.9831
% e1-cc2 0.0062
% ct_tox 0.8430
% fda 0.8508
% nr-ar 0.7822
% muv-466 0.8321

% \begin{table*}[h!]
%     \centering
%     \caption{Ablation study I: Performance when individual components of the \AWARE algorithm is removed.}
%     \vskip 0.15in
%     \begin{tabular}{| c | c | c | c | c | c | c |}
%         \hline
%         Task & Metric & Full & No $\Wv$ & No $\Ww$ & No $\Wg$ & Linear $\sigma$ \\
%         \toprule
%         \hline
%         delaney & RMSE & $0.6118$ & $0.7142$ & $0.6037$ & $0.6198$ & $0.9738$ \\
%         malaria & RMSE & $1.0635$ & $1.0868$ & $1.0432$ & $1.0745$ & $1.1292$ \\
%         qm7 & MAE & $41.6455$ & $41.6697$ & $39.5989$ & $46.9509$ & $73.1011$ \\
%         E1-CC2 & MAE & $0.0074$ & $0.0107$ & $0.0075$ & $0.0078$ & $0.0123$ \\
%         \hline
%         CT\_TOX & ROC & $0.8821$ & $0.8539$ & $0.8676$ & $0.8937$ & $0.8016$ \\
%         FDA\_APPROVED & ROC & $0.8657$ & $0.8397$ & $0.8388$ & $0.8617$ & $0.7852$ \\
%         NR-AR & ROC & $0.7722$ & $0.7854$ & $0.7710$ & $0.7687$ & $0.7785$ \\
%         MUV-466 & ROC & $0.7561$ & $0.6478$ & $0.6822$ & $0.7413$ & $0.7034$ \\
%         \hline
%     \end{tabular}
%     \label{tab:ablation1_performance_parts_removed}
% \end{table*}

% \begin{table*}[h!]
%     \centering
%     \caption{Ablation study I: Relative performance change when individual components of the {\AWARE} algorithm is removed compared to the full model. "+" means better performance and "-" means worse performance.}
%     \vskip 0.15in
%     \begin{tabular}{| c | c | c | c | c | c |}
%         \hline
%         Task & Metric & No $\Wv$ & No $\Ww$ & No $\Wg$ & Linear $\sigma$ \\
%         \toprule
%         \hline
%         \textsc{Delaney} & RMSE & $-16.74\%$ & $+1.32\%$ & $-1.31\%$ & $-59.17\%$ \\
%         \textsc{Malaria} & RMSE & $-2.19\%$ & $+1.91\%$ & $-1.03\%$ & $-6.18\%$ \\
%         \textsc{QM7} & MAE & $-0.06\%$ & $+4.91\%$ & $-12.74\%$ & $-75.53\%$ \\
%         \textsc{E1-CC2} & MAE & $-44.59\%$ & $-1.35\%$ & $-5.40\%$ & $-66.22\%$ \\
%         \hline
%         \textsc{CT\_TOX} & ROC & $-3.20\%$ & $-1.64\%$ & $+1.31\%$ & $-9.13\%$ \\
%         \textsc{FDA\_APPROVED} & ROC & $-3.00\%$ & $-3.11\%$ & $-0.46\%$ & $-9.30\%$ \\
%         \textsc{NR-AR} & ROC & $+1.71\%$ & $-0.16\%$ & $-0.45\%$ & $+0.82\%$ \\
%         \textsc{MUV-466} & ROC & $-14.32\%$ & $-9.77\%$ & $-1.96\%$ & $-6.97\%$ \\
%         \hline
%         average & & $-10.30\%$ & $-0.99\%$ & $-2.76\%$ & $-28.96\%$ \\
%         \hline
%     \end{tabular}
%     \label{tab:ablation1_performance_parts_removed}
% \end{table*}

==> tables/performance_extra_info_classification.tex <==
\begin{table*}[htb!]
    \centering
    \caption{Performance of models that use extra edge/3D information on classification tasks. The experiments are run on 5 different random seeds, and the average of the 5 reported for each task along with their standard deviation in the subscript. The best model in each task is highlighted in \hlblue{blue}. ROC-AUC is used as the evaluation metric. Higher is better.}
    % \vskip 0.15in
    \resizebox{0.5\textwidth}{!}{
    \begin{tabular}{ c  c  c  c }
        \toprule
        \textbf{Task} & \textbf{Weave} & \textbf{D-MPNN} & \textbf{{\AWARE}} \\
        \toprule
        \textsc{NR-AR} &  $0.774_{\pm 0.011}$ & $0.729_{\pm 0.057}$ & \best{0.786_{\pm 0.041}} \\
        \textsc{NR-AR-LBD} &  $0.824_{\pm 0.052}$ & $0.816_{\pm 0.079}$ & \best{0.865_{\pm 0.069}} \\
        \textsc{NR-AhR} &  $0.857_{\pm 0.020}$ & \best{0.892_{\pm 0.013}} & $0.884_{\pm 0.010}$ \\
        \textsc{NR-Aromatase} &  $0.827_{\pm 0.026}$ & $0.818_{\pm 0.039}$ & \best{0.861_{\pm 0.019}} \\
        \textsc{NR-ER} &  $0.736_{\pm 0.019}$ & $0.724_{\pm 0.035}$ & \best{0.760_{\pm 0.017}} \\
        \textsc{NR-ER-LBD} &  $0.809_{\pm 0.048}$ & $0.813_{\pm 0.040}$ & \best{0.851_{\pm 0.056}} \\
        \textsc{NR-PPAR-gamma} &  $0.803_{\pm 0.029}$ & $0.813_{\pm 0.046}$ & \best{0.862_{\pm 0.040}} \\
        \textsc{SR-ARE} &  $0.771_{\pm 0.032}$ & \best{0.833_{\pm 0.013}} & $0.827_{\pm 0.030}$ \\
        \textsc{SR-ATAD5} &  $0.765_{\pm 0.042}$ & $0.819_{\pm 0.050}$ & \best{0.841_{\pm 0.023}} \\
        \textsc{SR-HSE} &  $0.749_{\pm 0.043}$ & $0.753_{\pm 0.034}$ & \best{0.810_{\pm 0.023}} \\
        \textsc{SR-MMP} &  $0.886_{\pm 0.021}$ & $0.891_{\pm 0.018}$ & \best{0.905_{\pm 0.017}} \\
        \textsc{SR-p53} &  $0.787_{\pm 0.033}$ & $0.834_{\pm 0.019}$ & \best{0.841_{\pm 0.020}} \\
        \midrule
        \textsc{CT\_TOX} &  $0.844_{\pm 0.031}$ & $0.841_{\pm 0.068}$ & \best{0.905_{\pm 0.038}} \\
        \textsc{FDA\_APPROVED} &  $0.822_{\pm 0.074}$ & $0.881_{\pm 0.021}$ & \best{0.895_{\pm 0.050}} \\
        \midrule
        \textsc{HIV} &  $0.556_{\pm 0.059}$ & \best{0.831_{\pm 0.015}} & $0.823_{\pm 0.008}$ \\
        \midrule
        \textsc{MUV-466} &  $0.634_{\pm 0.148}$ & $0.776_{\pm 0.044}$ & \best{0.830_{\pm 0.078}} \\
        \textsc{MUV-548} &  $0.821_{\pm 0.071}$ & $0.932_{\pm 0.037}$ & \best{0.973_{\pm 0.011}} \\
        \textsc{MUV-600} &  $0.575_{\pm 0.148}$ & $0.559_{\pm 0.145}$ & \best{0.687_{\pm 0.062}} \\
        \textsc{MUV-644} &  $0.786_{\pm 0.089}$ & $0.806_{\pm 0.143}$ & \best{0.883_{\pm 0.060}} \\
        \textsc{MUV-652} &  $0.721_{\pm 0.133}$ & $0.539_{\pm 0.155}$ & \best{0.813_{\pm 0.107}} \\
        \textsc{MUV-689} &  $0.576_{\pm 0.300}$ & $0.620_{\pm 0.274}$ & \best{0.833_{\pm 0.077}} \\
        \textsc{MUV-692} &  $0.545_{\pm 0.166}$ & \best{0.654_{\pm 0.133}} & $0.574_{\pm 0.146}$ \\
        \textsc{MUV-712} &  $0.854_{\pm 0.065}$ & $0.797_{\pm 0.111}$ & \best{0.920_{\pm 0.050}} \\
        \textsc{MUV-713} &  $0.686_{\pm 0.116}$ & $0.593_{\pm 0.040}$ & \best{0.781_{\pm 0.151}} \\
        \textsc{MUV-733} &  \best{0.819_{\pm 0.101}} & $0.746_{\pm 0.153}$ & $0.819_{\pm 0.127}$ \\
        \textsc{MUV-737} &  $0.784_{\pm 0.033}$ & $0.805_{\pm 0.079}$ & \best{0.879_{\pm 0.077}} \\
        \textsc{MUV-810} &  $0.593_{\pm 0.165}$ & $0.665_{\pm 0.123}$ & \best{0.795_{\pm 0.120}} \\
        \textsc{MUV-832} &  $0.844_{\pm 0.128}$ & $0.946_{\pm 0.056}$ & \best{0.969_{\pm 0.021}} \\
        \textsc{MUV-846} &  $0.892_{\pm 0.058}$ & $0.870_{\pm 0.131}$ & \best{0.964_{\pm 0.027}} \\
        \textsc{MUV-852} &  $0.859_{\pm 0.060}$ & $0.785_{\pm 0.119}$ & \best{0.917_{\pm 0.090}} \\
        \textsc{MUV-858} &  $0.655_{\pm 0.155}$ & \best{0.749_{\pm 0.142}} & $0.657_{\pm 0.186}$ \\
        \textsc{MUV-859} &  $0.609_{\pm 0.150}$ & $0.465_{\pm 0.193}$ & \best{0.653_{\pm 0.186}} \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:clsfy_extra_info}
\end{table*}






% SEP 24
% \begin{table*}[htb!]
%     \centering
%     \caption{Performance of models that use extra edge/3D information on classification tasks. The experiments are run on 5 different random seeds and the average of the 5 reported for each task along with their standard deviation in the subscript. The best model in each task is highlighted in \hlblue{blue}. ROC-AUC is used as the evaluation metric. Higher is better.}
%     % \vskip 0.15in
%     \begin{tabular}{ c  c  c  c }
%         \toprule
%         Task & Weave & D-MPNN & {\AWARE} \\
%         \midrule
%         \textsc{NR-AR} & $0.774_{\pm 0.011}$ & $0.729_{\pm 0.057}$ & \best{0.798_{\pm 0.034}} \\
%         \textsc{NR-AR-LBD} & $0.824_{\pm 0.052}$ & $0.816_{\pm 0.079}$ & \best{0.865_{\pm 0.052}} \\
%         \textsc{NR-AhR} & $0.857_{\pm 0.020}$ & \best{0.892_{\pm 0.013}} & $0.887_{\pm 0.015}$ \\
%         \textsc{NR-Aromatase} & $0.827_{\pm 0.025}$ & $0.818_{\pm 0.039}$ & \best{0.858_{\pm 0.015}} \\
%         \textsc{NR-ER} & $0.736_{\pm 0.019}$ & $0.724_{\pm 0.035}$ & \best{0.766_{\pm 0.022}} \\
%         \textsc{NR-ER-LBD} & $0.809_{\pm 0.048}$ & $0.813_{\pm 0.040}$ & \best{0.848_{\pm 0.039}} \\
%         \textsc{NR-PPAR-gamma} & $0.803_{\pm 0.029}$ & $0.813_{\pm 0.046}$ & \best{0.875_{\pm 0.046}} \\
%         \textsc{SR-ARE} & $0.771_{\pm 0.032}$ & \best{0.833_{\pm 0.013}} & $0.822_{\pm 0.017}$ \\
%         \textsc{SR-ATAD5} & $0.765_{\pm 0.042}$ & $0.819_{\pm 0.050}$ & \best{0.849_{\pm 0.015}} \\
%         \textsc{SR-HSE} & $0.749_{\pm 0.043}$ & $0.753_{\pm 0.034}$ & \best{0.814_{\pm 0.024}} \\
%         \textsc{SR-MMP} & $0.886_{\pm 0.021}$ & $0.891_{\pm 0.018}$ & \best{0.904_{\pm 0.012}} \\
%         \textsc{SR-p53} & $0.787_{\pm 0.033}$ & $0.834_{\pm 0.019}$ & \best{0.850_{\pm 0.026}} \\
%         \midrule
%         \textsc{CT\_TOX} & $0.844_{\pm 0.031}$ & $0.841_{\pm 0.068}$ & \best{0.896_{\pm 0.019}} \\
%         \textsc{FDA\_APPROVED} & $0.822_{\pm 0.074}$ & $0.881_{\pm 0.021}$ & \best{0.886_{\pm 0.063}} \\
%         \midrule
%         \textsc{HIV} & $0.556_{\pm 0.059}$ & \best{0.831_{\pm 0.015}} & $0.825_{\pm 0.015}$ \\
%         \midrule
%         \textsc{MUV-466} & $0.634_{\pm 0.148}$ & $0.775_{\pm 0.044}$ & \best{0.783_{\pm 0.008}} \\
%         \textsc{MUV-548} & $0.821_{\pm 0.071}$ & $0.932_{\pm 0.037}$ & \best{0.974_{\pm 0.011}} \\
%         \textsc{MUV-600} & $0.575_{\pm 0.148}$ & $0.559_{\pm 0.145}$ & \best{0.680_{\pm 0.106}} \\
%         \textsc{MUV-644} & $0.786_{\pm 0.089}$ & $0.806_{\pm 0.143}$ & \best{0.869_{\pm 0.042}} \\
%         \textsc{MUV-652} & $0.721_{\pm 0.133}$ & $0.539_{\pm 0.155}$ & \best{0.810_{\pm 0.146}} \\
%         \textsc{MUV-689} & $0.576_{\pm 0.300}$ & $0.620_{\pm 0.274}$ & \best{0.802_{\pm 0.189}} \\
%         \textsc{MUV-692} & $0.545_{\pm 0.166}$ & $0.654_{\pm 0.133}$ & \best{0.656_{\pm 0.190}} \\
%         \textsc{MUV-712} & $0.854_{\pm 0.065}$ & $0.797_{\pm 0.111}$ & \best{0.922_{\pm 0.030}} \\
%         \textsc{MUV-713} & $0.686_{\pm 0.116}$ & $0.593_{\pm 0.040}$ & \best{0.772_{\pm 0.113}} \\
%         \textsc{MUV-733} & \best{0.819_{\pm 0.101}} & $0.746_{\pm 0.153}$ & $0.789_{\pm 0.108}$ \\
%         \textsc{MUV-737} & $0.784_{\pm 0.033}$ & $0.805_{\pm 0.079}$ & \best{0.897_{\pm 0.049}} \\
%         \textsc{MUV-810} & $0.593_{\pm 0.165}$ & $0.665_{\pm 0.123}$ & \best{0.787_{\pm 0.079}} \\
%         \textsc{MUV-832} & $0.844_{\pm 0.128}$ & $0.946_{\pm 0.056}$ & \best{0.966_{\pm 0.023}} \\
%         \textsc{MUV-846} & $0.892_{\pm 0.058}$ & $0.870_{\pm 0.130}$ & \best{0.969_{\pm 0.029}} \\
%         \textsc{MUV-852} & $0.859_{\pm 0.060}$ & $0.785_{\pm 0.119}$ & \best{0.932_{\pm 0.072}} \\
%         \textsc{MUV-858} & $0.654_{\pm 0.155}$ & \best{0.749_{\pm 0.142}} & $0.657_{\pm 0.111}$ \\
%         \textsc{MUV-859} & $0.609_{\pm 0.150}$ & $0.465_{\pm 0.193}$ & \best{0.653_{\pm 0.098}} \\
%         \bottomrule
%     \end{tabular}
%     \label{tab:clsfy_extra_info}
% \end{table*}

% \begin{table*}[htb!]
%     \centering
%     \caption{Performance of models that use extra edge/3D information on classification tasks. The experiments are run on five different random seeds and the average of the five reported for each task along with their standard deviation in the subscript. The best model in each task is highlighted in \sethlcolor{lightblue}\hl{\textbf{blue}}. Higher is better.}
%     \vskip 0.15in
%     \begin{tabular}{| c | c | c | c |}
%         \hline
%         Task & Weave & D-MPNN & {\AWARE} \\
%         \toprule
%         \hline
%         \textsc{NR-AR} & $0.7739_{\pm 0.0108}$ & $0.7288_{\pm 0.0573}$ & \best{0.7981_{\pm 0.0343}} \\
%         \textsc{NR-AR-LBD} & $0.8240_{\pm 0.0519}$ & $0.8162_{\pm 0.0791}$ & \best{0.8655_{\pm 0.0521}} \\
%         \textsc{NR-AhR} & $0.8570_{\pm 0.0203}$ & \best{0.8922_{\pm 0.0131}} & $0.8875_{\pm 0.0151}$ \\
%         \textsc{NR-Aromatase} & $0.8267_{\pm 0.0255}$ & $0.8184_{\pm 0.0390}$ & \best{0.8580_{\pm 0.0153}} \\
%         \textsc{NR-ER} & $0.7362_{\pm 0.0193}$ & $0.7245_{\pm 0.0354}$ & \best{0.7665_{\pm 0.0219}} \\
%         \textsc{NR-ER-LBD} & $0.8090_{\pm 0.0482}$ & $0.8131_{\pm 0.0400}$ & \best{0.8478_{\pm 0.0393}} \\
%         \textsc{NR-PPAR-gamma} & $0.8035_{\pm 0.0292}$ & $0.8129_{\pm 0.0462}$ & \best{0.8750_{\pm 0.0458}} \\
%         \textsc{SR-ARE} & $0.7706_{\pm 0.0324}$ & \best{0.8327_{\pm 0.0134}} & $0.8220_{\pm 0.0172}$ \\
%         \textsc{SR-ATAD5} & $0.7652_{\pm 0.0420}$ & $0.8186_{\pm 0.0497}$ & \best{0.8494_{\pm 0.0155}} \\
%         \textsc{SR-HSE} & $0.7488_{\pm 0.0427}$ & $0.7527_{\pm 0.0337}$ & \best{0.8137_{\pm 0.0242}} \\
%         \textsc{SR-MMP} & $0.8859_{\pm 0.0210}$ & $0.8914_{\pm 0.0176}$ & \best{0.9044_{\pm 0.0125}} \\
%         \textsc{SR-p53} & $0.7866_{\pm 0.0330}$ & $0.8340_{\pm 0.0189}$ & \best{0.8504_{\pm 0.0265}} \\
%         \hline
%         \textsc{CT\_TOX} & $0.8437_{\pm 0.0313}$ & $0.8406_{\pm 0.0676}$ & \best{0.8959_{\pm 0.0191}} \\
%         \textsc{FDA\_APPROVED} & $0.8221_{\pm 0.0740}$ & \best{0.8808_{\pm 0.0213}} & $0.8860_{\pm 0.0634}$ \\
%         \hline
%         \textsc{HIV} & $0.5560_{\pm 0.0593}$ & \best{0.8312_{\pm 0.0150}} & $0.8253_{\pm 0.0146}$ \\
%         \hline
%         \textsc{MUV-466} & $0.6337_{\pm 0.1481}$ & $0.7755_{\pm 0.0440}$ & \best{0.7829_{\pm 0.0085}} \\
%         \textsc{MUV-548} & $0.8209_{\pm 0.0710}$ & $0.9322_{\pm 0.0366}$ & \best{0.9745_{\pm 0.0114}} \\
%         \textsc{MUV-600} & $0.5751_{\pm 0.1478}$ & $0.5590_{\pm 0.1453}$ & \best{0.6800_{\pm 0.1062}} \\
%         \textsc{MUV-644} & $0.7865_{\pm 0.0886}$ & $0.8063_{\pm 0.1433}$ & \best{0.8687_{\pm 0.0423}} \\
%         \textsc{MUV-652} & $0.7215_{\pm 0.1329}$ & $0.5386_{\pm 0.1550}$ & \best{0.8097_{\pm 0.1460}} \\
%         \textsc{MUV-689} & $0.5759_{\pm 0.3001}$ & $0.6199_{\pm 0.2744}$ & \best{0.8018_{\pm 0.1888}} \\
%         \textsc{MUV-692} & $0.5448_{\pm 0.1660}$ & $0.6540_{\pm 0.1333}$ & \best{0.6561_{\pm 0.1901}} \\
%         \textsc{MUV-712} & $0.8538_{\pm 0.0651}$ & $0.7973_{\pm 0.1113}$ & \best{0.9220_{\pm 0.0305}} \\
%         \textsc{MUV-713} & $0.6865_{\pm 0.1158}$ & $0.5933_{\pm 0.0403}$ & \best{0.7717_{\pm 0.1131}} \\
%         \textsc{MUV-733} & \best{0.8195_{\pm 0.1013}} & $0.7458_{\pm 0.1527}$ & $0.7888_{\pm 0.1078}$ \\
%         \textsc{MUV-737} & $0.7842_{\pm 0.0334}$ & $0.8053_{\pm 0.0788}$ & \best{0.8970_{\pm 0.0490}} \\
%         \textsc{MUV-810} & $0.5929_{\pm 0.1654}$ & $0.6654_{\pm 0.1233}$ & \best{0.7872_{\pm 0.0786}} \\
%         \textsc{MUV-832} & $0.8436_{\pm 0.1284}$ & $0.9465_{\pm 0.0556}$ & \best{0.9661_{\pm 0.0235}} \\
%         \textsc{MUV-846} & $0.8920_{\pm 0.0579}$ & $0.8697_{\pm 0.1305}$ & \best{0.9686_{\pm 0.0286}} \\
%         \textsc{MUV-852} & $0.8588_{\pm 0.0597}$ & $0.7846_{\pm 0.1187}$ & \best{0.9322_{\pm 0.0720}} \\
%         \textsc{MUV-858} & $0.6545_{\pm 0.1549}$ & \best{0.7487_{\pm 0.1420}} & $0.6574_{\pm 0.1114}$ \\
%         \textsc{MUV-859} & $0.6093_{\pm 0.1505}$ & $0.4652_{\pm 0.1935}$ & \best{0.6526_{\pm 0.0979}} \\
%         \hline
%     \end{tabular}
%     \label{tab:clsfy_extra_info}
% \end{table*}

==> tables/performance_extra_info_regression.tex <==
\begin{table*}[ht!]
    \centering
    \caption{Performance of models that use extra edge/3D information on regression tasks. The experiments are run on 5 different random seeds, and the average of the 5 reported for each task along with their standard deviation in the subscript. Since only \textsc{QM8} and \textsc{QM9} tasks include 3D information, DTNN and MPNN are evaluated only on those. The top-3 models in each task are highlighted in \hlgray{gray} and the best one is highlighted in \hlblue{blue}. RMSE is used as the evaluation metric for the first three tasks and MAE for the rest. Lower is better.}
    % \vskip 0.15in
    \resizebox{0.6\textwidth}{!}{
    \begin{tabular}{c  c  c  c  c  c }
        \toprule
        \textbf{Task} & \textbf{Weave} & \textbf{DTNN} & \textbf{MPNN} & \textbf{D-MPNN} & \textbf{{\AWARE}} \\
        \toprule
        \textsc{Delaney} & \topthree{0.620_{\pm 0.121}} & -- & -- & \topthree{0.696_{\pm 0.065}} & \best{0.589_{\pm 0.051}} \\
        \midrule
        \textsc{Malaria} & \topthree{1.471_{\pm 0.071}} & -- & -- & \topthree{1.070_{\pm 0.025}} & \best{1.061_{\pm 0.036}} \\
        \midrule
        \textsc{CEP} & \topthree{2.573_{\pm 0.292}} & -- & -- & \best{1.116_{\pm 0.048}} & \topthree{1.252_{\pm 0.023}} \\
        \midrule
        \textsc{QM7} & \topthree{59.690_{\pm 3.075}} & -- & -- & \topthree{68.938_{\pm 5.893}} & \best{40.304_{\pm 3.670}} \\
        \midrule
        \textsc{E1-CC2} & \topthree{0.007_{\pm 0.001}} & $0.007_{\pm 0.000}$ & \best{0.006_{\pm 0.000}} & \topthree{0.006_{\pm 0.000}} & $0.007_{\pm 0.000}$ \\
        \textsc{E2-CC2} & $0.008_{\pm 0.000}$ & \topthree{0.007_{\pm 0.000}} & \best{0.007_{\pm 0.000}} & \topthree{0.007_{\pm 0.001}} & $0.008_{\pm 0.000}$ \\
        \textsc{f1-CC2} & \topthree{0.018_{\pm 0.001}} & $0.022_{\pm 0.001}$ & $0.020_{\pm 0.001}$ & \topthree{0.014_{\pm 0.001}} & \best{0.013_{\pm 0.000}} \\
        \textsc{f2-CC2} & \topthree{0.035_{\pm 0.001}} & $0.041_{\pm 0.000}$ & $0.039_{\pm 0.001}$ & \topthree{0.031_{\pm 0.001}} & \best{0.030_{\pm 0.002}} \\
        \textsc{E1-PBE0} & \topthree{0.007_{\pm 0.001}} & \best{0.006_{\pm 0.001}} & $0.007_{\pm 0.002}$ & $0.007_{\pm 0.001}$ & \topthree{0.007_{\pm 0.000}} \\
        \textsc{E2-PBE0} & \topthree{0.007_{\pm 0.000}} & \topthree{0.007_{\pm 0.000}} & \best{0.006_{\pm 0.000}} & $0.008_{\pm 0.001}$ & $0.008_{\pm 0.000}$ \\
        \textsc{f1-PBE0} & \topthree{0.015_{\pm 0.002}} & $0.018_{\pm 0.001}$ & $0.018_{\pm 0.002}$ & \topthree{0.012_{\pm 0.001}} & \best{0.011_{\pm 0.000}} \\
        \textsc{f2-PBE0} & \topthree{0.027_{\pm 0.002}} & $0.034_{\pm 0.001}$ & $0.032_{\pm 0.002}$ & \topthree{0.024_{\pm 0.001}} & \best{0.023_{\pm 0.000}} \\
        \textsc{E1-CAM} & $0.006_{\pm 0.000}$ & \topthree{0.006_{\pm 0.000}} & \best{0.006_{\pm 0.000}} & \topthree{0.006_{\pm 0.001}} & $0.006_{\pm 0.000}$ \\
        \textsc{E2-CAM} & \topthree{0.006_{\pm 0.000}} & $0.007_{\pm 0.000}$ & \topthree{0.006_{\pm 0.000}} & \best{0.006_{\pm 0.000}} & $0.007_{\pm 0.000}$ \\
        \textsc{f1-CAM} & \topthree{0.016_{\pm 0.001}} & $0.019_{\pm 0.001}$ & $0.019_{\pm 0.001}$ & \topthree{0.012_{\pm 0.001}} & \best{0.012_{\pm 0.001}} \\
        \textsc{f2-CAM} & \topthree{0.030_{\pm 0.002}} & $0.036_{\pm 0.001}$ & $0.034_{\pm 0.002}$ & \topthree{0.026_{\pm 0.000}} & \best{0.024_{\pm 0.001}} \\
        \midrule
        \textsc{mu} & $0.617_{\pm 0.013}$ & \best{0.244_{\pm 0.006}} & \topthree{0.283_{\pm 0.072}} & \topthree{0.464_{\pm 0.013}} & $0.535_{\pm 0.007}$ \\
        \textsc{alpha} & \topthree{0.680_{\pm 0.076}} & \best{0.387_{\pm 0.043}} & $0.696_{\pm 0.094}$ & \topthree{0.408_{\pm 0.026}} & $0.774_{\pm 0.035}$ \\
        \textsc{homo} & $0.005_{\pm 0.000}$ & \best{0.003_{\pm 0.000}} & \topthree{0.004_{\pm 0.000}} & \topthree{0.003_{\pm 0.000}} & $0.006_{\pm 0.000}$ \\
        \textsc{lumo} & $0.005_{\pm 0.000}$ & \topthree{0.003_{\pm 0.000}} & \topthree{0.004_{\pm 0.000}} & \best{0.003_{\pm 0.000}} & $0.005_{\pm 0.000}$ \\
        \textsc{gap} & $0.007_{\pm 0.000}$ & \topthree{0.005_{\pm 0.000}} & \topthree{0.006_{\pm 0.000}} & \best{0.005_{\pm 0.000}} & $0.007_{\pm 0.000}$ \\
        \textsc{r2} & \topthree{33.679_{\pm 2.587}} & \best{10.485_{\pm 2.982}} & \topthree{26.759_{\pm 14.689}} & $41.083_{\pm 4.077}$ & $83.000_{\pm 8.780}$ \\
        \textsc{zpve} & $0.001_{\pm 0.000}$ & \topthree{0.000_{\pm 0.000}} & $0.002_{\pm 0.001}$ & \best{0.000_{\pm 0.000}} & \topthree{0.001_{\pm 0.000}} \\
        \textsc{cv} & \topthree{0.254_{\pm 0.025}} & \best{0.125_{\pm 0.032}} & $0.280_{\pm 0.092}$ & \topthree{0.173_{\pm 0.006}} & $0.586_{\pm 0.042}$ \\
        \textsc{u0} & $2.419_{\pm 1.339}$ & \topthree{1.429_{\pm 0.558}} & $3.478_{\pm 3.140}$ & \topthree{0.673_{\pm 1.024}} & \best{0.090_{\pm 0.017}} \\
        \textsc{u298} & $1.375_{\pm 0.245}$ & \topthree{0.880_{\pm 0.344}} & $2.665_{\pm 3.479}$ & \topthree{0.557_{\pm 0.791}} & \best{0.086_{\pm 0.009}} \\
        \textsc{h298} & $1.472_{\pm 0.221}$ & \topthree{0.959_{\pm 0.424}} & $1.189_{\pm 0.421}$ & \topthree{0.522_{\pm 0.708}} & \best{0.098_{\pm 0.007}} \\
        \textsc{g298} & $1.948_{\pm 0.691}$ & \topthree{0.809_{\pm 0.356}} & $1.264_{\pm 0.413}$ & \topthree{0.581_{\pm 0.555}} & \best{0.086_{\pm 0.010}} \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:reg_extra_info}
\end{table*}










% SEP 24
% \begin{table*}[ht!]
%     \centering
%     \caption{Performance of models that use extra edge/3D information on regression tasks. The experiments are run on 5 different random seeds and the average of the 5 reported for each task along with their standard deviation in the subscript. Since only \textsc{QM8} and \textsc{QM9} tasks include 3D information, DTNN and MPNN are evaluated only on those. The top-3 models in each task are highlighted in \hlgray{gray} and the best one is highlighted in \hlblue{blue}. RMSE is used as the evaluation metric for the first three tasks and MAE for the rest. Lower is better.}
%     % \vskip 0.15in
%     \begin{tabular}{c  c  c  c  c  c }
%         \toprule
%         Task & Weave & DTNN & MPNN & D-MPNN & {\AWARE} \\
%         \midrule
%         \textsc{Delaney} & \topthree{0.620_{\pm 0.121}} & -- & -- & \topthree{0.696_{\pm 0.064}} & \best{0.589_{\pm 0.051}} \\
%         \midrule
%         \textsc{Malaria} & \topthree{1.471_{\pm 0.071}} & -- & -- & \topthree{1.070_{\pm 0.025}} & \best{1.061_{\pm 0.036}} \\
%         \midrule
%         \textsc{CEP} & \topthree{2.573_{\pm 0.292}} & -- & -- & \best{1.116_{\pm 0.048}} & \topthree{1.252_{\pm 0.023}} \\
%         \midrule
%         \textsc{QM7} & \topthree{59.690_{\pm 3.075}} & -- & -- & \topthree{68.938_{\pm 5.893}} & \best{40.304_{\pm 3.670}} \\
%         \midrule
%         \textsc{E1-CC2} & \topthree{0.006_{\pm 0.001}} & $0.007_{\pm 0.000}$ & \best{0.006_{\pm 0.000}} & \topthree{0.006_{\pm 0.000}} & $0.007_{\pm 0.000}$ \\
%         \textsc{E2-CC2} & $0.007_{\pm 0.000}$ & \topthree{0.007_{\pm 0.000}} & \best{0.007_{\pm 0.000}} & \topthree{0.007_{\pm 0.000}} & $0.008_{\pm 0.000}$ \\
%         \textsc{f1-CC2} & \topthree{0.018_{\pm 0.001}} & $0.022_{\pm 0.001}$ & $0.020_{\pm 0.001}$ & \topthree{0.014_{\pm 0.001}} & \best{0.013_{\pm 0.000}} \\
%         \textsc{f2-CC2} & \topthree{0.035_{\pm 0.001}} & $0.041_{\pm 0.000}$ & $0.039_{\pm 0.001}$ & \topthree{0.031_{\pm 0.001}} & \best{0.030_{\pm 0.002}} \\
%         \textsc{E1-PBE0} & \topthree{0.007_{\pm 0.001}} & \best{0.006_{\pm 0.001}} & $0.007_{\pm 0.002}$ & $0.007_{\pm 0.001}$ & \topthree{0.007_{\pm 0.000}} \\
%         \textsc{E2-PBE0} & \topthree{0.007_{\pm 0.000}} & \topthree{0.007_{\pm 0.000}} & \best{0.006_{\pm 0.000}} & $0.008_{\pm 0.001}$ & $0.008_{\pm 0.000}$ \\
%         \textsc{f1-PBE0} & \topthree{0.015_{\pm 0.002}} & $0.018_{\pm 0.001}$ & $0.018_{\pm 0.002}$ & \topthree{0.012_{\pm 0.001}} & \best{0.011_{\pm 0.000}} \\
%         \textsc{f2-PBE0} & \topthree{0.027_{\pm 0.001}} & $0.034_{\pm 0.001}$ & $0.032_{\pm 0.002}$ & \topthree{0.024_{\pm 0.001}} & \best{0.023_{\pm 0.000}} \\
%         \textsc{E1-CAM} & $0.006_{\pm 0.000}$ & \topthree{0.006_{\pm 0.000}} & \best{0.005_{\pm 0.000}} & \topthree{0.006_{\pm 0.000}} & $0.006_{\pm 0.000}$ \\
%         \textsc{E2-CAM} & \topthree{0.006_{\pm 0.000}} & $0.007_{\pm 0.000}$ & \topthree{0.006_{\pm 0.000}} & \best{0.006_{\pm 0.000}} & $0.007_{\pm 0.000}$ \\
%         \textsc{f1-CAM} & \topthree{0.016_{\pm 0.001}} & $0.019_{\pm 0.001}$ & $0.019_{\pm 0.001}$ & \topthree{0.012_{\pm 0.001}} &\best{0.012_{\pm 0.001}} \\
%         \textsc{f2-CAM} & \topthree{0.030_{\pm 0.002}} & $0.036_{\pm 0.001}$ & $0.034_{\pm 0.002}$ & \topthree{0.026_{\pm 0.000}} & \best{0.024_{\pm 0.001}} \\
%         \midrule
%         \textsc{mu} & $0.617_{\pm 0.013}$ & \best{0.244_{\pm 0.005}} & \topthree{0.283_{\pm 0.072}} & \topthree{0.464_{\pm 0.013}} & $0.535_{\pm 0.007}$ \\
%         \textsc{alpha} & \topthree{0.680_{\pm 0.076}} & \best{0.387_{\pm 0.043}} & $0.696_{\pm 0.094}$ & \topthree{0.408_{\pm 0.025}} & $0.774_{\pm 0.035}$ \\
%         \textsc{homo} &  $0.005_{\pm 0.000}$ & \best{0.003_{\pm 0.000}} & \topthree{0.004_{\pm 0.000}} & \topthree{0.003_{\pm 0.000}} & $0.006_{\pm 0.000}$ \\
%         \textsc{lumo} & $0.005_{\pm 0.000}$ & \topthree{0.003_{\pm 0.000}} & \topthree{0.004_{\pm 0.000}} & \best{0.003_{\pm 0.000}} & $0.005_{\pm 0.000}$ \\
%         \textsc{gap} & $0.007_{\pm 0.000}$ & \topthree{0.005_{\pm 0.000}} & \topthree{0.006_{\pm 0.000}} & \best{0.005_{\pm 0.000}} & $0.007_{\pm 0.000}$ \\
%         \textsc{r2} & \topthree{33.679_{\pm 2.587}} & \best{10.485_{\pm 2.982}} & \topthree{26.759_{\pm 14.689}} & $41.083_{\pm 4.077}$ & $83.000_{\pm 8.780}$ \\
%         \textsc{zpve} & $0.001_{\pm 0.000}$ & \topthree{0.000_{\pm 0.000}} & $0.002_{\pm 0.001}$ & \best{0.000_{\pm 0.000}} & \topthree{0.001_{\pm 0.000}} \\
%         \textsc{cv} & \topthree{0.254_{\pm 0.025}} & \best{0.124_{\pm 0.031}} & $0.280_{\pm 0.092}$ & \topthree{0.173_{\pm 0.006}} & $0.586_{\pm 0.042}$ \\
%         \textsc{u0} & $2.419_{\pm 1.339}$ & \topthree{1.429_{\pm 0.558}} & $3.478_{\pm 3.140}$ & \topthree{0.673_{\pm 1.024}} & \best{0.090_{\pm 0.017}} \\
%         \textsc{u298} & $1.375_{\pm 0.245}$ & \topthree{0.880_{\pm 0.344}} & $2.665_{\pm 3.479}$ & \topthree{0.557_{\pm 0.791}} & \best{0.086_{\pm 0.009}} \\
%         \textsc{h298} & $1.472_{\pm 0.221}$ & \topthree{0.959_{\pm 0.424}} & $1.189_{\pm 0.421}$ & \topthree{0.522_{\pm 0.708}} & \best{0.098_{\pm 0.007}} \\
%         \textsc{g298} & $1.948_{\pm 0.690}$ & \topthree{0.809_{\pm 0.356}} & $1.264_{\pm 0.413}$ & \topthree{0.581_{\pm 0.555}} & \best{0.086_{\pm 0.010}} \\
%         \bottomrule
%     \end{tabular}
%     \label{tab:reg_extra_info}
% \end{table*}

% \begin{table*}[ht!]
%     \centering
%     \caption{Performance of models that use extra edge/3D information on regression tasks. The experiments are run on 5 different random seeds and the average of the 5 reported for each task along with their standard deviation in the subscript. Since only \textsc{QM8} and \textsc{QM9} tasks include 3D information, DTNN and MPNN are evaluated only on those. The top-3 models in each task are highlighted in \hlgray{gray} and the best one is highlighted in \hlblue{blue}. RMSE is used as the evaluation metric for the first three tasks and MAE for the rest. Lower is better.}
%     % \vskip 0.15in
%     \begin{tabular}{c  c  c  c  c  c }
%         \toprule
%         Task & Weave & DTNN & MPNN & D-MPNN & {\AWARE} \\
%         \midrule
%         \textsc{Delaney} & \topthree{0.620_{\pm 0.121}} & -- & -- & \topthree{0.696_{\pm 0.064}} & \best{0.587_{\pm 0.055}} \\
%         \midrule
%         \textsc{Malaria} & \topthree{1.471_{\pm 0.071}} & -- & -- & \topthree{1.070_{\pm 0.025}} & \best{1.060_{\pm 0.027}} \\
%         \midrule
%         \textsc{CEP} & \topthree{2.573_{\pm 0.292}} & -- & -- & \best{1.116_{\pm 0.048}} & \topthree{1.264_{\pm 0.019}} \\
%         \midrule
%         \textsc{QM7} & \topthree{59.690_{\pm 3.075}} & -- & -- & \topthree{68.938_{\pm 5.893}} & \best{40.947_{\pm 2.703}} \\
%         \midrule
%         \textsc{E1-CC2} & \topthree{0.006_{\pm 0.001}} & $0.007_{\pm 0.000}$ & \best{0.006_{\pm 0.000}} & \topthree{0.006_{\pm 0.000}} & $0.007_{\pm 0.000}$ \\
%         \textsc{E2-CC2} & $0.007_{\pm 0.000}$ & \topthree{0.007_{\pm 0.000}} & \best{0.007_{\pm 0.000}} & \topthree{0.007_{\pm 0.000}} & $0.008_{\pm 0.000}$ \\
%         \textsc{f1-CC2} & \topthree{0.018_{\pm 0.001}} & $0.022_{\pm 0.001}$ & $0.020_{\pm 0.001}$ & \topthree{0.014_{\pm 0.001}} & \best{0.013_{\pm 0.000}} \\
%         \textsc{f2-CC2} & \topthree{0.035_{\pm 0.001}} & $0.041_{\pm 0.000}$ & $0.039_{\pm 0.001}$ & \topthree{0.031_{\pm 0.001}} & \best{0.029_{\pm 0.001}} \\
%         \textsc{E1-PBE0} & \topthree{0.007_{\pm 0.001}} & \best{0.006_{\pm 0.001}} & $0.007_{\pm 0.002}$ & $0.007_{\pm 0.001}$ & \topthree{0.006_{\pm 0.000}} \\
%         \textsc{E2-PBE0} & \topthree{0.007_{\pm 0.000}} & \topthree{0.007_{\pm 0.000}} & \best{0.006_{\pm 0.000}} & $0.008_{\pm 0.001}$ & $0.007_{\pm 0.000}$ \\
%         \textsc{f1-PBE0} & \topthree{0.015_{\pm 0.002}} & $0.018_{\pm 0.001}$ & $0.018_{\pm 0.002}$ & \topthree{0.012_{\pm 0.001}} & \best{0.011_{\pm 0.000}} \\
%         \textsc{f2-PBE0} & \topthree{0.027_{\pm 0.001}} & $0.034_{\pm 0.001}$ & $0.032_{\pm 0.002}$ & \topthree{0.024_{\pm 0.001}} & \best{0.023_{\pm 0.001}} \\
%         \textsc{E1-CAM} & $0.006_{\pm 0.000}$ & \topthree{0.006_{\pm 0.000}} & \best{0.005_{\pm 0.000}} & \topthree{0.006_{\pm 0.000}} & $0.006_{\pm 0.000}$ \\
%         \textsc{E2-CAM} & \topthree{0.006_{\pm 0.000}} & $0.007_{\pm 0.000}$ & \topthree{0.006_{\pm 0.000}} & \best{0.006_{\pm 0.000}} & $0.007_{\pm 0.000}$ \\
%         \textsc{f1-CAM} & \topthree{0.016_{\pm 0.001}} & $0.019_{\pm 0.001}$ & $0.019_{\pm 0.001}$ & \topthree{0.012_{\pm 0.001}} &\best{0.012_{\pm 0.000}} \\
%         \textsc{f2-CAM} & \topthree{0.030_{\pm 0.002}} & $0.036_{\pm 0.001}$ & $0.034_{\pm 0.002}$ & \topthree{0.026_{\pm 0.000}} & \best{0.025_{\pm 0.001}} \\
%         \midrule
%         \textsc{mu} & $0.617_{\pm 0.013}$ & \best{0.244_{\pm 0.005}} & \topthree{0.283_{\pm 0.072}} & \topthree{0.464_{\pm 0.013}} & $0.529_{\pm 0.008}$ \\
%         \textsc{alpha} & \topthree{0.680_{\pm 0.076}} & \best{0.387_{\pm 0.043}} & $0.696_{\pm 0.094}$ & \topthree{0.408_{\pm 0.025}} & $0.775_{\pm 0.024}$ \\
%         \textsc{homo} &  $0.005_{\pm 0.000}$ & \best{0.003_{\pm 0.000}} & \topthree{0.004_{\pm 0.000}} & \topthree{0.003_{\pm 0.000}} & $0.005_{\pm 0.000}$ \\
%         \textsc{lumo} & $0.005_{\pm 0.000}$ & \topthree{0.003_{\pm 0.000}} & \topthree{0.004_{\pm 0.000}} & \best{0.003_{\pm 0.000}} & $0.005_{\pm 0.000}$ \\
%         \textsc{gap} & $0.007_{\pm 0.000}$ & \topthree{0.005_{\pm 0.000}} & \topthree{0.006_{\pm 0.000}} & \best{0.005_{\pm 0.000}} & $0.007_{\pm 0.000}$ \\
%         \textsc{r2} & \topthree{33.679_{\pm 2.587}} & \best{10.485_{\pm 2.982}} & \topthree{26.759_{\pm 14.689}} & $41.083_{\pm 4.077}$ & $94.898_{\pm 7.853}$ \\
%         \textsc{zpve} & $0.001_{\pm 0.000}$ & \topthree{0.000_{\pm 0.000}} & $0.002_{\pm 0.001}$ & \best{0.000_{\pm 0.000}} & \topthree{0.001_{\pm 0.000}} \\
%         \textsc{cv} & \topthree{0.254_{\pm 0.025}} & \best{0.124_{\pm 0.031}} & $0.280_{\pm 0.092}$ & \topthree{0.173_{\pm 0.006}} & $0.534_{\pm 0.029}$ \\
%         \textsc{u0} & $2.419_{\pm 1.339}$ & \topthree{1.429_{\pm 0.558}} & $3.478_{\pm 3.140}$ & \topthree{0.673_{\pm 1.024}} & \best{0.078_{\pm 0.018}} \\
%         \textsc{u298} & $1.375_{\pm 0.245}$ & \topthree{0.880_{\pm 0.344}} & $2.665_{\pm 3.479}$ & \topthree{0.557_{\pm 0.791}} & \best{0.070_{\pm 0.009}} \\
%         \textsc{h298} & $1.472_{\pm 0.221}$ & \topthree{0.959_{\pm 0.424}} & $1.189_{\pm 0.421}$ & \topthree{0.522_{\pm 0.708}} & \best{0.092_{\pm 0.014}} \\
%         \textsc{g298} & $1.948_{\pm 0.690}$ & \topthree{0.809_{\pm 0.356}} & $1.264_{\pm 0.413}$ & \topthree{0.581_{\pm 0.555}} & \best{0.073_{\pm 0.011}} \\
%         \bottomrule
%     \end{tabular}
%     \label{tab:reg_extra_info}
% \end{table*}

% \begin{table*}[ht!]
%     \centering
%     \caption{Performance of models that use extra edge/3D information on regression tasks. The experiments are run on five different random seeds and the average of the five reported for each task along with their standard deviation in the subscript. The top-3 models in each task are highlighted in \sethlcolor{lightlightgray}\hl{gray} and the best one is highlighted in \sethlcolor{lightblue}\hl{\textbf{blue}}. Lower is better.}
%     \vskip 0.15in
%     \begin{tabular}{| c | c | c | c | c | c |}
%         \hline
%         Task & Weave & DTNN & MPNN & D-MPNN & {\AWARE} \\
%         \toprule
%         \hline
%         \textsc{Delaney} & \topthree{0.6203_{\pm 0.1214}} & -- & -- & \topthree{0.6960_{\pm 0.0645}} & \best{0.5873_{\pm 0.0554}} \\
%         \textsc{Malaria} & \topthree{1.4707_{\pm 0.0709}} & -- & -- & \topthree{1.0697_{\pm 0.0254}} & \best{1.0597_{\pm 0.0271}} \\
%         \textsc{CEP} & \topthree{2.5735_{\pm 0.2917}} & -- & -- & \best{1.1164_{\pm 0.0480}} & \topthree{1.2640_{\pm 0.0190}} \\
%         \textsc{QM7} & \topthree{59.6899_{\pm 3.0748}} & -- & -- & \topthree{68.9378_{\pm 5.8927}} & \best{40.9474_{\pm 2.7030}} \\
%         \hline
%         \textsc{E1-CC2} & \topthree{0.0065_{\pm 0.0006}} & $0.0066_{\pm 0.0003}$ & \best{0.0058_{\pm 0.0003}} & \topthree{0.0062_{\pm 0.0003}} & $0.0066_{\pm 0.0002}$ \\
%         \textsc{E2-CC2} & $0.0075_{\pm 0.0004}$ & \topthree{0.0075_{\pm 0.0002}} & \best{0.0073_{\pm 0.0005}} & \topthree{0.0075_{\pm 0.0005}} & $0.0080_{\pm 0.0001}$ \\
%         \textsc{f1-CC2} & \topthree{0.0183_{\pm 0.0012}} & $0.0216_{\pm 0.0008}$ & $0.0199_{\pm 0.0015}$ & \topthree{0.0142_{\pm 0.0008}} & \best{0.0131_{\pm 0.0004}} \\
%         \textsc{f2-CC2} & \topthree{0.0352_{\pm 0.0012}} & $0.0413_{\pm 0.0004}$ & $0.0387_{\pm 0.0014}$ & \topthree{0.0307_{\pm 0.0009}} & \best{0.0294_{\pm 0.0007}} \\
%         \textsc{E1-PBE0} & \topthree{0.0066_{\pm 0.0007}} & \best{0.0062_{\pm 0.0006}} & $0.0069_{\pm 0.0023}$ & $0.0068_{\pm 0.0014}$ & \topthree{0.0063_{\pm 0.0003}} \\
%         \textsc{E2-PBE0} & \topthree{0.0066_{\pm 0.0001}} & \topthree{0.0068_{\pm 0.0002}} & \best{0.0064_{\pm 0.0004}} & $0.0077_{\pm 0.0010}$ & $0.0074_{\pm 0.0002}$ \\
%         \textsc{f1-PBE0} & \topthree{0.0153_{\pm 0.0016}} & $0.0182_{\pm 0.0009}$ & $0.0177_{\pm 0.0017}$ & \topthree{0.0121_{\pm 0.0010}} & \best{0.0112_{\pm 0.0005}} \\
%         \textsc{f2-PBE0} & \topthree{0.0270_{\pm 0.0015}} & $0.0340_{\pm 0.0010}$ & $0.0321_{\pm 0.0021}$ & \topthree{0.0241_{\pm 0.0009}} & \best{0.0226_{\pm 0.0007}} \\
%         \textsc{E1-CAM} & $0.0059_{\pm 0.0004}$ & \topthree{0.0057_{\pm 0.0002}} & \best{0.0055_{\pm 0.0004}} & \topthree{0.0057_{\pm 0.0005}} & $0.0062_{\pm 0.0002}$ \\
%         \textsc{E2-CAM} & \topthree{0.0063_{\pm 0.0004}} & $0.0066_{\pm 0.0004}$ & \topthree{0.0063_{\pm 0.0003}} & \best{0.0062_{\pm 0.0002}} & $0.0071_{\pm 0.0002}$ \\
%         \textsc{f1-CAM} & \topthree{0.0163_{\pm 0.0009}} & $0.0194_{\pm 0.0006}$ & $0.0192_{\pm 0.0009}$ & \topthree{0.0124_{\pm 0.0006}} &\best{0.0121_{\pm 0.0003}} \\
%         \textsc{f2-CAM} & \topthree{0.0303_{\pm 0.0016}} & $0.0357_{\pm 0.0007}$ & $0.0340_{\pm 0.0025}$ & \topthree{0.0257_{\pm 0.0003}} & \best{0.0251_{\pm 0.0014}} \\
%         \hline
%         \textsc{mu} & $0.6174_{\pm 0.0132}$ & \best{0.2438_{\pm 0.0055}} & \topthree{0.2832_{\pm 0.0724}} & \topthree{0.4644_{\pm 0.0129}} & $0.5286_{\pm 0.0084}$ \\
%         \textsc{alpha} & \topthree{0.6798_{\pm 0.0764}} & \best{0.3869_{\pm 0.0433}} & $0.6964_{\pm 0.0942}$ & \topthree{0.4081_{\pm 0.0255}} & $0.7755_{\pm 0.0245}$ \\
%         \textsc{homo} &  $0.0050_{\pm 0.0002}$ & $0.0035_{\pm 0.0001}$ & $0.0040_{\pm 0.0001}$ & $0.0035_{\pm 0.0001}$ & $0.0052_{\pm 0.0001}$ \\
%         \textsc{lumo} & $0.0051_{\pm 0.0002}$ & \topthree{0.0035_{\pm 0.0001}} & \topthree{0.0042_{\pm 0.0002}} & \best{0.0033_{\pm 0.0000}} & $0.0048_{\pm 0.0001}$ \\
%         \textsc{gap} & $0.0074_{\pm 0.0004}$ & \topthree{0.0054_{\pm 0.0002}} & \topthree{0.0061_{\pm 0.0002}} & \best{0.0050_{\pm 0.0003}} & $0.0071_{\pm 0.0002}$ \\
%         \textsc{r2} & \topthree{33.6793_{\pm 2.5869}} & \best{10.4847_{\pm 2.9821}} & \topthree{26.7587_{\pm 14.6890}} & $41.0829_{\pm 4.0768}$ & $94.8979_{\pm 7.8532}$ \\
%         \textsc{zpve} & $0.0009_{\pm 0.0003}$ & \topthree{0.0004_{\pm 0.0001}} & $0.0016_{\pm 0.0007}$ & \best{0.0004_{\pm 0.0001}} & \topthree{0.0007_{\pm 0.0000}} \\
%         \textsc{cv} & \topthree{0.2537_{\pm 0.0253}} & \best{0.1245_{\pm 0.0315}} & $0.2800_{\pm 0.0916}$ & \topthree{0.1732_{\pm 0.0061}} & $0.5344_{\pm 0.0287}$ \\
%         \textsc{u0} & $2.4186_{\pm 1.3393}$ & \topthree{1.4286_{\pm 0.5580}} & $3.4784_{\pm 3.1404}$ & \topthree{0.6732_{\pm 1.0240}} & \best{0.0785_{\pm 0.0183}} \\
%         \textsc{u298} & $1.3752_{\pm 0.2452}$ & \topthree{0.8800_{\pm 0.3439}} & $2.6646_{\pm 3.4790}$ & \topthree{0.5566_{\pm 0.7915}} & \best{0.0696_{\pm 0.0087}} \\
%         \textsc{h298} & $1.4719_{\pm 0.2213}$ & \topthree{0.9594_{\pm 0.4241}} & $1.1887_{\pm 0.4206}$ & \topthree{0.5221_{\pm 0.7080}} & \best{0.0925_{\pm 0.0140}} \\
%         \textsc{g298} & $1.9482_{\pm 0.6905}$ & \topthree{0.8091_{\pm 0.3559}} & $1.2643_{\pm 0.4127}$ & \topthree{0.5812_{\pm 0.5546}} & \best{0.0731_{\pm 0.0114}} \\
%         \hline
%     \end{tabular}
%     \label{tab:reg_extra_info}
% \end{table*}

==> tables/table2.tex <==
\begin{table*}[th!]
    \centering
    \caption{Performance on several tasks from both molecular and social network domains. The top-3 and best performing models for each task are highlighted in \hlgray{gray} and \hlblue{blue}, respectively.}
    % \vskip 0.15in
    \resizebox{\textwidth}{!}{
    \begin{tabular}{ l  c  c  c c  c  c  c  c  c  c }
        \toprule
        \textbf{Task} & \textbf{Metric} & \textbf{Morgan FP} & \textbf{WL Kernel} & \textbf{GCNN} & \textbf{GAT} & \textbf{GIN} & \textbf{Attentive FP} & \textbf{PNA} & \textbf{N-Gram Graph} &
        \textbf{{\AWARE}} \\
        \midrule
        \textsc{IMDB-BINARY} & ACC & -- & $0.680_{\pm 0.022}$ & $0.698_{\pm 0.026}$ & $0.568_{\pm 0.047}$ & $0.696_{\pm 0.037}$ & \topthree{0.716_{\pm 0.022}} & \topthree{0.710_{\pm 0.011}} & $0.522_{\pm 0.036}$ & \best{0.740_{\pm 0.020}} \\
        \textsc{REDDIT-BINARY} & ACC & -- & $0.892_{\pm 0.017}$	& $0.931_{\pm 0.013}$ & $0.900_{\pm 0.036}$ & \topthree{0.933_{\pm 0.009}} & $0.864_{\pm 0.029}$ & \topthree{0.938_{\pm 0.010}} & $0.764_{\pm 0.026}$ & \best{0.949_{\pm 0.014}} \\
        \textsc{COLLAB} & ACC & -- & $0.567_{\pm 0.011}$ & $0.660_{\pm 0.009}$ & $0.616_{\pm 0.029}$ & \topthree{0.669_{\pm 0.014}} & $0.653_{\pm 0.012}$ & \topthree{0.675_{\pm 0.024}} & $0.376_{\pm 0.119}$ & \best{0.739_{\pm 0.017}} \\
        \midrule
        \textsc{CT\_TOX} & ROC & $0.813_{\pm 0.036}$ & $0.830_{\pm 0.057}$ & $0.860_{\pm 0.027}$ & $0.828_{\pm 0.075}$ & $0.859_{\pm 0.063}$ & \topthree{0.873_{\pm 0.053}} & \topthree{0.895_{\pm 0.043}} & $0.849_{\pm 0.024}$ & \best{0.905_{\pm 0.038}} \\
        \textsc{FDA\_APPROVED} & ROC & $0.795_{\pm 0.084}$ & $0.862_{\pm 0.029}$ & $0.866_{\pm 0.028}$ & \best{0.899_{\pm 0.033}} & \topthree{0.883_{\pm 0.025}} & $0.870_{\pm 0.070}$ & $0.879_{\pm 0.022}$ & $0.852_{\pm 0.044}$ & \topthree{0.895_{\pm 0.050}} \\
        \midrule
        \textsc{Delaney} & RMSE & $1.081_{\pm 0.073}$ & $1.160_{\pm 0.050}$ & $0.762_{\pm 0.151}$ & $0.954_{\pm 0.151}$ & $0.840_{\pm 0.070}$ & \topthree{0.615_{\pm 0.026}} & $0.922_{\pm 0.122}$ & \topthree{0.744_{\pm 0.068}} & \best{0.585_{\pm 0.042}} \\
        \textsc{QM7} & MAE & $118.883_{\pm 2.421}$ & $173.582_{\pm 4.293}$ & $76.000_{\pm 2.743}$ & $213.014_{\pm 10.618}$ & $82.681_{\pm 3.979}$ & \topthree{74.710_{\pm 9.079}} & $108.913_{\pm 25.555}$ & \topthree{49.661_{\pm 4.246}} & \best{39.697_{\pm 3.400}} \\
        \bottomrule
    \end{tabular}
    }
    \label{tab:table2}
\end{table*}
